ChannelComp: A General Method for Computation by Communications

Over-the-air computation (AirComp) is a well-known technique by which several wireless devices transmit by analog amplitude modulation to achieve a sum of their transmit signals at a common receiver. The underlying physical principle is the superposition property of the radio waves. Since such superposition is analog and in amplitude, it is natural that AirComp uses analog amplitude modulations. Unfortunately, this is impractical because most wireless devices today use digital modulations. It would be highly desirable to use digital communications because of their numerous benefits, such as error correction, synchronization, acquisition of channel state information, and widespread use. However, when we use digital modulations for AirComp, a general belief is that the superposition property of the radio waves returns a meaningless overlapping of the digital signals. In this paper, we break through such beliefs and propose an entirely new digital channel computing method named ChannelComp, which can use digital as well as analog modulations. We propose a feasibility optimization problem that ascertains the optimal modulation for computing arbitrary functions over-the-air. Additionally, we propose pre-coders to adapt existing digital modulation schemes for computing the function over the multiple access channel. The simulation results verify the superior performance of ChannelComp compared to AirComp, particularly for the product functions, with more than 10 dB improvement of the computation error.

==> Algorithm/Alg_Nestrove.tex <==
\begin{algorithm}[!th]
\caption{Nesterov SCA algorithm for the maximizing the minimum distance}\label{alg:SCA}
\begin{algorithmic}[1]
	\State \textbf{Input:} Function $f(x_1,\ldots,x_K),\epsilon_{SCA}. \mu$,
	\State set $N = q^K$, $M = q K$
	\State Initialize randomly  $\bm{x}^{(0)}$ such that $\|\bm{x}^{(0)}\|_2^2\leq P$
	\State \textbf{Output:} Modulation vector $\bm{x} \in \mathbb{C}^{N}$
	\Procedure{First Order Method}{$\{f_i\}_{i=1}^{N}, \sigma$}
	\For {$t \gets 1,2,\ldots,$}
	\State Compute $\bm{c}_{i,j}^{(t)} = 2 \tilde{\bm{B}}_{i,j} \bm{x}^{(t-1)}$
	\State Compute $\bm{d}_{i,j}^{(t)} = \bm{x}^{(t-1) \mathsf{H}}\tilde{\bm{B}}_{i,j} \bm{x}^{(t-1)} - \log(\tfrac{|f_i-f_j|}{2})$
	\State Compute $\bm{x}^{t} = \underset{\|\bm{x}\|_2^2\leq P}{\rm argmin}~\upsilon_{\mu}(\bm{x}, \bm{c}_{i,j}^{(t)},\bm{d}_{i,j}^{(t)}) $ using a first order method
	\If{The objective value is below $\epsilon_{SCA}$}
	\State $\bm{x}^* = \bm{x}^t$
	\State break
	\EndIf
	\EndFor
	\EndProcedure
\end{algorithmic}
\end{algorithm}

==> Tables/Tab_Comparison,tex <==
\begin{table}[!t]
\centering
\begin{tabular}{|c| c| }
\toprule
\textbf{Variable} & \textbf{Interpretation} \\
\midrule
$\mathcal{D}_{f}$ & Domain set of function $f$ \\ 
$\mathscr{E}_k(\cdot)$ &  encoder at node $k$ \\
$f$ &  Desired function \\
$f^{(i)}$ & Value of output  $i$ of desired function $f$ \\
 $h_k$ & Channel coefficient between node $k$ and the center point  \\
 $K$ & Number of nodes in the network \\
 $q$ & Number of quantization level \\
 $\mathcal{R}_f$ &  Range set of function $f$ \\
 $\mathcal{R}_s$ &   Set of all possible constellation points \\
 $\vec{s}_i$ & The induced value over-the-air corresponding to $f^{(i)}$ \\  
 $\mathscr{T}(\cdot)$ & Tabular mapping to compute function $f$ \\
 $\vec{x}_k$ & Modulated signal of node $k$\\
 $\vec{y}$ & The received value at the center point \\
 $\vec{z}$ & Additive white Gaussian noise \\
\bottomrule
\end{tabular}
\caption{Reference list of commonly used variables in this survey. Ordered alphabetically and by case.}
\label{Tab:List}
\end{table}
